InFact: Informativeness Alignment for Improved LLM Factuality

Factual completeness is a general term that captures how detailed and informative a factually correct text is. For instance, the factual sentence ``Barack Obama was born in the United States'' is factually correct, though less informative than the factual sentence ``Barack Obama was born in Honolulu, Hawaii, United States''. Despite the known fact that LLMs tend to hallucinate and generate factually incorrect text, they might also tend to choose to generate factual text that is indeed factually correct and yet less informative than other, more informative choices. In this work, we tackle this problem by proposing an informativeness alignment mechanism. This mechanism takes advantage of recent factual benchmarks to propose an informativeness alignment objective. This objective prioritizes answers that are both correct and informative. A key finding of our work is that when training a model to maximize this objective or optimize its preference, we can improve not just informativeness but also factuality.

==> 02_rules.tex <==

\section{Completeness Rules}

In this section, we describe each of the factual completeness rules we defined, which we will later use to generate our dataset. 

\subsection{Rules Formulation}

Recall that a world fact can be described via a triplet $(s, r, o)$, while $s$ is the subject world entity, $o$ is the object world entity, and $r$ is a well-defined relation between them. For example - (Paris, capital of, France) and (Lily-Rose Depp, father, Johnny Depp). For clearer formulation, we first define the following:

\begin{enumerate}
    \item \textbf{General type of world entity}: Given a world entity $e$, we define its general type, and denote it by $GT(e)$ as the general instance type of $e$ such as: Human, Place, Date, Animal, Book, Work, etc. 

    \item \textbf{Specific type of world entity}: Given a world entity $e$, we define its general type, and denote it by $ST(e)$ as the a more specific type which is also $GT(e)$. For example, $ST(e)$ can be city, hospital, year, 
\end{enumerate}

We denote a completeness rule with $w$. Each of the rules is associated to one or more factual relations, $R_w = \{r_1, ..., r_m\}$, and essentially define the structure of the most complete answer we expect for a factual question related to $r \in R_w$. Specifically, each rule defines a set of concepts $C_w = \{c_1, ..., c_{N_w}\}$, such that when a model is asked a factual question related to $r \in R_w$, the most complete answer one expects must include all $c_1, ..., c_{N_w}$, while $N_w$ is the number of concepts in $C_w$. Each concept is essentially a specific type of world entity. 

\subsection{Set of Rules}

We next describe the rules we have defined to generate our dataset.

\paragraph{Place of birth} 

==> 03_data.tex <==

\section{Dataset}

In this section, we elaborate on the structure of our proposed dataset, as well as on the curation pipeline. We additionally report several statistics about the dataset and about its data quality.

\subsection{General Structure}
\label{sec:dataset_structure}

Intuitively, our dataset is a collection of questions, and for each question, we define a hierarchy of possible answers. Each of the possible answers belongs to a specific level in the hierarchy. Level 1 includes the most "complete" answers, as level $L_i$ includes the least "complete" but still correct answers ($L_i$ refers to the number of levels in the hierarchy of answers that corresponds to question $i$). 
More formally, we denote our dataset with $\mathcal{D} = \{(q_i, H_i)\}_{i = 1}^{N}$, and $H_i = \{A_j = \{a_1, ..., a_{b_j}\}\}_{j = 1}^{L_i}$, while $N$ stands for the number of examples in the dataset, $q_i$ for the $i$th question in the dataset, $H_i$ for its corresponds hierarchy of answers, and $A_j$ for the $j$th level in this hierarchy which is essentially a set includes all the possible answers of this level. 


\subsection{Data Generation Pipeline}

\subsection{Data Statistics}

\subsection{Data Quality}




==> Tables/ablation_no_structure_tuning.tex <==




\begin{table*}[t]
\setlength{\belowcaptionskip}{-4pt}
% \setlength\tabcolsep{2.5pt}
% \footnotesize
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}l  cc  ccc  cc@{}}
\toprule
&  \multicolumn{2}{c}{GRANOLA QA} & \multicolumn{3}{c}{QAMPARI} &  \multicolumn{2}{c}{RoMEQA} \\ 
 % [0.1cm]
\cmidrule(r){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-8}
\multicolumn{1}{c}{} & \textbf{Accuracy}  & \textbf{Informativeness}  & \textbf{P} & \textbf{R} & \textbf{F1}  & \textbf{F1}  & \textbf{$F1^{R}$}  \\
\midrule
\texttt{\llamaoneb + informativeness-alignment but no structure tuning}     & $48.1$    &$48.1$   &$48.1$  
                    & $35.0$    &$35.0$   &$35.0$ 
                    & $29.5$    &$29.5$   &$29.5$   \\
\texttt{\llamaoneb + informativeness-alignment}  & $51.8$    &$40.8$   &$-$  
                    & $34.1$    &$22.8$   &$-$ 
                    & $39.4$    &$21.0$   &$-$   \\ \midrule
\texttt{\llamathreeb + informativeness-alignment but no structure tunin}     & $60.4$    &$38.3$   &$-$ 
                    & $42.9$    &$25.1$ &$-$ 
                    & $45.8$    &$14.9$ &$-$ \\ 
\texttt{\llamathreeb + informativeness-alignment}    & $54.4$    &$40.5$   &$-$ 
                    & $39.6$    &$22.0$ &$-$ 
                    & $44.4$    &$20.7$ &$-$ \\ \midrule
\texttt{\llamaeightb + informativeness-alignment but no structure tunin}    & $52.8$    &$41.0$   &$-$ 
                    & $41.2$    &$21.9$ &$-$ 
                    & $44.9$    &$21.1$ &$-$  \\
\textbf{\llamaeightb + informativeness-alignment} & $\mathbf{63.8}$    &$40.6$   &$-$
                            & $47.6$    &$31.0$   &$-$   
                            & $49.8$    &$24.5$   &$-$   \\

\bottomrule
\end{tabular}
}
% \end{center}
\caption{}. 
\label{table:ablation_no_structure_tuning}
\end{table*}
% \vspace{5mm}



